Eliom: A Language for Modular Tierless Web Programming

Tierless Web programming languages allow programmers to combine client-side and server-side programming in a single program. Programmers can then define components with both client and server parts and get flexible, efficient and typesafe client-server communications. However, the expressive client-server features found in most tierless languages are not necessarily compatible with functionalities found in many mainstream languages. In particular, we would like to benefit from type safety, an efficient execution, static compilation, modularity and separate compilation. In this paper, we propose Eliom, an industrial-strength tierless functional Web programming language which extends OCaml with support for rich client/server interactions. It allows to build whole applications as a single distributed program, in which it is possible to define modular tierless libraries with both server and client behaviors and combine them effortlessly. Eliom is the only language that combines type-safe and efficient client/server communications with a static compilation model that supports separate compilation and modularity. It also supports excellent integration with OCaml, allowing to transparently leverage its ecosystem. To achieve all these features, Eliom borrows ideas not only from distributed programming languages, but also from meta-programming and modern module systems. We present the design of Eliom, how it can be used in practice and its formalization; including its type system, semantics and compilation scheme. We show that this compilation scheme preserves typing and semantics, and that it supports separate compilation.

==> theory/core/grammar.tex <==

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../../main"
%%% End:

\begin{subfigure}[t]{0.48\linewidth}
\begin{align*}
  \htag{Locations}
  \loc ::=&\ s\ |\ c\ |\ \base\tag{Core}\\
  \mloc ::=&\ \sideX\ |\ \loc\tag{Mixed}\\
  \htag{Path}
  p ::=&\ x_i\ |\ p.x\ |\ \appm{p_1}{p_2}\\
  \htag{Expressions}
  e ::=&\ c\ |\ v_i\ |\ \Y\ |\ \app{e}{e}\ |\ \lam{v}{e}\\
  |&\ \letin{v}{e}{e}\tag{Let}\\
  |&\ p.v \tag{Path}\\
  |&\ \cv{ e } \tag{Fragments}\\
  |&\ \injf{v}{f} \tag{Injections}\\[2mm]
  f ::= &\ p.v\ |\ v_i\ |\ c \tag{Converter}\\
  c \in&\ \Const_\loc \tag{Constants}
\end{align*}
\end{subfigure}\quad
\begin{subfigure}[t]{0.48\linewidth}
  \begin{align*}
  \htag{Environments}
    \Env ::=&\ \emptyEnv\\
    |&\ \Env;\bindingm{x}{M} \tag{Module}\\
    |&\ \Env;\binding{v}{\sigma} \tag{Value}\\
    |&\ \Env;\bindingty{t}{\tau} \tag{Type}\\
    |&\ \Env;\bindingabs{t} \tag{Abstract Type}\\
  \htag{Type Schemes}
  \sigma ::=&\ \forall\alpha_{\loc_i}^*.\tau\\
  \htag{Type Expressions}
  \tau ::=&\ \alpha_\loc\ |\ \lamtype{\tau}{\tau}\ |\ \type{t_i}\\
    |&\ p.t \tag{Path}\\
    |&\ \cvtype{\tau} \tag{Fragments}\\
    |&\ \conv{\tau}{\tau} \tag{Converters}
\end{align*}
\end{subfigure}


==> theory/core/subdefineloc.tex <==
\begin{align*}
  \canbedefloc{\sideX&}{s}&
  \canbedefloc{\sideX&}{c}&
  \canbedefloc{\sideX&}{\base}&
  \forall \mloc \in \{s,c,\sideX,\base\}\ \canbedefloc{\mloc&}{\mloc}
\end{align*}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> theory/core/subloc.tex <==
\begin{align*}
  \canuseloc{\sideX&}{s}&
  \canuseloc{\sideX&}{c}&
  \canuseloc{\base&}{s}&
  \canuseloc{\base&}{c}&
  \canuseloc{\base&}{\sideX}&
  \forall \mloc \in \{s,c,\sideX,\base\}\ \canuseloc{\mloc&}{\mloc}
\end{align*}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> theory/datatypegrammar.tex <==
\begin{align*}
  \tag{Programs}
  p ::=&\ \typem{\appty{\alpha_{\loc_i}^*}{t}}{\tau_\loc};\ p\ |\ \dots\\
  \tag{Types}
  \tau ::=&\ \appty{\tau_i^*}{t}\ |\ \dots\\
  \tag{Environments}
  \Env ::=&\ \Env;\bindingabs{\appty{\alpha_{\loc_i}^*}{t}}\ |
            \ \Env;\bindingty{\appty{\alpha_{\loc_i}^*}{t}}{\tau_\loc}\ |\ \dots
\end{align*}
%
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> theory/datatypevalidity.tex <==
%
\textbf{Type Expression Validity Rules}
\begin{mathpar}
  \inferrule[Constr]
  { i \in {1,\dots,n} \\
    \bindingabs{\appty{\alpha_{\loc_i}^n}{t}} \in \Env \\
    \forall i, \wf[\loc_i]{\Env}{\tau_i}
  }
  { \wf{\Env}{\appty{\tau_i^n}{t}} }
\end{mathpar}
\textbf{Program Typing Rules}
\begin{mathpar}
  \inferrule[TypeDecl]
  { \wf{\Env}{\tau} \\
    \ftv{\tau} = \{\alpha_{\loc_1},\dots,\alpha_{\loc_n}\} \\
    \wtp{\Env;\bindingty{\appty{\alpha_{\loc_i}^n}{t}}{\tau}}{p}{\tau'}
  }
  { \wtp{\Env}{\typem{\appty{\alpha_{\loc_i}^n}{t}}{\tau};\ p}{\tau'} }
\end{mathpar}
\textbf{Type Equivalence}
\begin{mathpar}
  \inferrule[ParamTypeAbsEq]
  { \bindingty[\loc']{\appty{\alpha_{\loc_i}^n}{t}}{\tau}\in\Env \\
    \added{\canuseloc{\loc'}{\loc}} \\
    \equivty{\Env}{\subst[\loci]{\alpha_\loci}{\tau_i}{\tau}_n}{\tau'}
  }
  { \equivty{\Env}{\appty{\tau_i^n}{t}}{\tau'} }
  \and
  \inferrule[ParamTypeEq]
  { \bindingabs[\loc']{\appty{\alpha_{\loc_i}^n}{t}}\in\Env \\
    \added{\canuseloc{\loc'}{\loc}} \\
    \forall i \in\rg{1}{n},\ \equivty[\loc_i]{\Env}{\tau_i}{\tau'_i}
  }
  { \equivty{\Env}{\appty{\tau_i^n}{t}}{\appty{{\tau'_i}^n}{t}} }
\end{mathpar}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> theory/discussion.tex <==
\subsection{Discussion around mixed functors}
\label{sec:discussion}

In this thesis, we presented the notion of ``mixed functors'', which
are functors that take as argument and return mixed module composed
of both client and server code. As we saw, those functors,
while quite expressive, have several limitations. In this
section, we will try to explore a little bit the design
space around mixed functors and which limitations we think
could be lifted.

First, let us recall the design constraints of \eliom: typing
and slicing are done statically and separate
compilation is supported. This prevents us from ``erasing'' functors
by inlining them and also prevents us from dynamically
generating the code contained in functors. Furthermore, we want to support
languages extensions such as \ocaml, where functor application
can depend on the control flow (notably, first class modules).

% Mixed functors can be seen from two perspectives. The client part of a mixed
% functor is exactly the same as a pure client functor. Indeed, since we disallow
% arbitrary injections, we can remove all the server code and leave the client
% part untouched.
% The server part, however, can be seen as a pair of a server module and
% an client module hidden inside a fragment. Indeed, given the presence of
% fragments inside the server part, each mixed functor application done on the
% server needs a corresponding functor application on the client which performs
% all the client-side evaluation. This means that we need a way to associate each
% server version of mixed modules to its client version.
% In order to do that, we equip the server version with a new field $\dyn$
% which contains a unique identifier. This identifier is later transmitted to the
% client and used to retrieve the client part of the mixed module.

% In order to handle functors, we register each mixed functor application that
% happens on the server and use $\dyn$ fields to perform them client side.
% Since mixed functors can only be applied to mixed structures, they necessarily
% have a $\dyn$ field.

One alternative solution would be \emph{fully separable} functors: mixed functors such that client and server execution
are completely independent.
While this would be easy to implement, it would also mean preventing any meaningful
usage of fragments inside functors.
Our version of mixed functors is slightly more expressive:
the client part of the functor is indeed independent from the server part, but
the server part is not.
The cost is that we must do some extra book-keeping to ensure that for each
server-side application of a mixed functors, all the client side effects are performed.
We believe this expressive power is sufficient for most use cases.
%
There are however several limitations to our approach, which we shall discuss point-by-point
now.

\paragraph{Mixed functors arguments}

An important restriction of mixed functors is that their arguments can only be mixed
structures. The reason for this restriction is that the $\dyn$ field is used in
order to keep track of client applications from the server. In the semantics
presented in this thesis, the $\dyn$ field is represented simply as a regular
structure field, which means only structures can be passed as argument.
A first step would be to allow a similar field to be added to functors.
While it is a bit delicate to formalize, it should be possible to
implement it in \ocaml by simply adding an additional field to the closure.
%
A second step would be to allow base, client and server modules as arguments. As with
usual mixed functors, care must be taken during typechecking to not specialize
eagerly. Given that this constraint is respected, one possibility would be
to introduce a new module-level operation that can take a base, server or client
structure and turn it into a mixed structure.
Given a client module \eliomc{A}, this could be done
by inserting a structure of the form \eliomc{(struct include\%client A end)}.
This could even be done transparently, since the location of modules is always known.

\paragraph{Injections}

Injections inside mixed functors can only refer to identifiers outside of the functor.
This restriction seems particularly difficult to lift, as demonstrated
by the example in \cref{sec:functor}. One would need to evaluate the usefulness of
mixed functors in first-class contexts. It might be possible to
rewrite usages of injections to escaped values in fragments. In all cases, these
changes would be invasive and of limited usefulness.

\paragraph{Sliceability constraints}\label{sec:compilation:lift}

The sliceability requirement presented in \cref{sec:compilation:sliceability} is quite
restrictive.
Its goal is to ensure that
$\pbind_m$ expressions are not nested and that module references are unique.
This requirement can be relaxed in different manners. For mixed structures without
functors, this requirements can be completely removed trivially, since internal
modules are known.

For functors, there are two possibilities. A first idea would be to apply lambda-lifting
to functors. By simply lifting mixed functors to the outer scope, we ensure that
$\pbind$ operations are noted nested. Another possibility would be to use a similar
technique to the one used for fragments inside functors: by prefixing each statically
generated reference with the locally available $\dyn$ field, we ensure
uniqueness while allowing arbitrary nesting.

\paragraph{Double application of the client side of mixed functors}

As mentioned in \cref{sec:eliom:execution:functor}, the client-side part
of a mixed functor, when applied in a mixed context, might be called twice.
While this is not so problematic in the context of applicative and pure functors,
it might prove more troublesome with generative or impure functors.
This problem is difficult to solve in general.
In particular, it is in fairly direct conflict with the design decision, justified by \cref{sec:functor}, to make the client and server side of a mixed
functor application independent.
One potential solution would be to provide
a special interpretation of mixed application in mixed contexts that would ensure
that the result of the client-side functor application is properly reused.
Notably, this might be doable by generating at compile time an identifier
for each known returned client module.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:

%  LocalWords:  sliceability


==> theory/eliom.tex <==
\subsection{Syntax}
\label{sec:eliom:syntax}

The syntax is presented in \cref{eliom:grammar}. It extends the syntax
presented in \cref{ml:grammar}.

\subsubsection{Expression language}

The expression language is extended with two new constructs: fragments
and injections.
%
A {\em client fragment} $\cv{e}$ can be used on the server to
represent an expression that will be computed on the client,
but whose future value can be manipulated on the server.
%
An {\em injection} $\injf{v}{f}$ can be used on the client to
access values defined on the server. An injection must make explicit
use of a converter $f$ that specifies how to send the value. In
particular, this should involve a serialization step, executed on the
server, followed by a deserialization step executed on the client.
%
For ease of presentation, injections are only done on variables and
constants.
In the implementation, this restriction is removed by adding
a lifting transformation.
For clarity, we sometimes distinguish injections \emph{per se}, which occur outside
of fragments, and escaped values, which occur inside fragments.

The syntax of types is also extended with two constructs. A {\em fragment type} $\cvtype{\tau}$ is the type of a fragment.
A {\em converter type} $\conv{\tau_s}{\tau_c}$ is the type of a converter taking
a server value of type $\tau_s$ and returning a client value of type $\tau_c$.
%
All type variables $\alpha_\loc$ are annotated with a core
location $\loc$. There are now three sets of constants: client, server and base.

\subsubsection{Module language}

The main change in the module language of \etiny is that structure and signature
components are annotated
with locations. Value and type declarations can be annotated with a core location $\loc$
which is either $\base$, $s$ or $c$.
Module declarations can also have one additional possible location: the mixed location $\sideX$.
Only modules on location $\sideX$ can have subfields on different locations.
%
We also introduce mixed functors, noted $\functor[\sideX]{X}{\Mm}{\Mm}$, which body can
contain both client and server declarations.
%
A program is a list of declarations including a client value declaration $\ret$ which is the result of the program.

\subsection{Type system}\label{sec:eliom:type}

Judgments are now annotated with a location that specifies where the given
code should be typechecked. Judgments on the expression language can accept
any core location $\loc$ while module judgments accept mixed locations $\mloc$.
%
We note $\Typeof_\loc(c)$ the type of a given constant $c$ on the location $\loc$.
%
Binding in typing environments, just like in signatures, are annotated with
a location.
The first three kind of bindings, corresponding to the core language, can only
appear on core locations: $s$, $c$ or $b$.
Modules can also be of mixed location $\sideX$.
Names are namespaced by locations, which means it is valid to have both a client
and a server value with both the same name.

\subsubsection{Expressions}

The new typing rules for expressions are presented in
\cref{core:typing,core:validity,core:eqtype}.
We introduce two typing rules for the new constructions.
%
Rule \mysc{Fragment} is for the construction of client fragments and can only be applied on the server.
If $e$ is of type $\tau$ {\em on the client}, then $\cv{e}$ is of type $\cvtype{\tau}$ {\em on the server}.
%
Rule \mysc{Injection} is for the communication from the server to the client
and can only be applied on the client.
If $e$ is of type $\tau_s$ on the server and $f$ is of type $\conv{\tau_s}{\tau_c}$ on the server,
then $\injf{e}{f}$ is of type $\tau_c$ on the client.
%
Since no other typing rules involves client fragments, it is
impossible to deconstruct them.

The last difference with usual \ml rules are the visibility of variable.
As described earlier, bindings in \emodule are located. Since access across
sides are explicit,
we want to prevent the use of client variables on the server, for example.
In rule \mysc{Var}, to use on location $\loc$ the variable $v$ which is bound on location $\loc'$,
we check that $\canuseloc{\loc'}{\loc}$, defined in \cref{loc:canuse}, which means
that the definition on $\loc$ can be used in $\loc'$.
Base elements $\base$ are usable everywhere. Mixed elements $\sideX$ are
usable in both client and server.
Type variables are also annotated with a location and follow the same rules.
Using type variables from the client on the server, for example,
is disallowed.

The validity judgement on types presented in \cref{core:validity} is extended to check
that locations are respected both for type constructors and type variables. This
judgement is used in type declaration, which are presented in the module system.

\begin{figure}[!p]
  \renewcommand\added\addedx
  \renewcommand\addedrule\addedno
  \input{theory/core/typing}\vspace{-3mm}
  \caption{\etiny expression typing rules -- $\wt{\Env}{e}{\tau}$}
  \label{core:typing}
  \input{theory/core/validity}\vspace{-3mm}
  \caption{Type validity rules -- $\wf{\Env}{\tau}$}
  \label{core:validity}
\end{figure}

\begin{figure}[htb]
  \renewcommand\added\addedx
  \renewcommand\addedrule\addedno
  \input{theory/core/equivty}\vspace{-3mm}
  \caption{Type equivalence rules -- $\equivty{\Env}{\tau}{\tau'}$}
  \label{core:eqtype}
\end{figure}

\subsubsection{Converters}\label{sec:converter}

To transmit values from the server to the client, we need a
serialization format. We assume the existence of a type $\serial$ in
$\Const_b$ which represents the
serialization format. The actual format is irrelevant. For instance,
one could use JSON or XML.

Converters are special values that describe how to move a value from the server to the client.
A converter can be understood as a pair of functions.
%
A converter $f$ of type $\conv{\tau_s}{\tau_c}$ is composed of a
server-side encoding function of type $\lamtype{\tau_s}{\serial}$, and
a client-side decoding function of type $\lamtype{\serial}{\tau_c}$.
%
We assume the existence of two built-in converters:
\begin{itemize}[noitemsep]
\item The $\serial$ converter of type $\conv{\serial}{\serial}$. Both sides are the identity.
\item The $\fragment$ converter of type  $\forall\alpha_c.(\conv{\cvtype{\alpha_c}}{\alpha_c})$.
\end{itemize}


\subsubsection{Type universes}\label{sec:typeuniv}

It is important to note that there is no identity converter (of type $\forall\alpha.(\conv{\alpha}{\alpha})$). Indeed the client and server type universes
are distinct and we cannot translate arbitrary types from one to the other.
%
Some types are only available on one side: database handles, system types, \js API types.
%
Some types, while available on both sides
(because they are in base for example), are simply not transferable.
For example, functions cannot be serialized in general.
Another example is file handles: they are available both on the server and
on the client, but moving a file handle from server to client seems adventurous.

Finally, some types may share a semantic meaning, but not their actual representation. This is the case where converters are used, as demonstrated in \cref{tuto:heterogeneous}.

\subsubsection{Mixed datatypes}
\label{sec:datatypes}

In \cref{sec:ml:datatypes,sec:ml:module}, we saw that the version of \ml
we consider supports an interesting
combination of three features: abstract datatypes, parametrized datatypes and
separate compilation at the module level.
\etiny, as an extension of \ml, also supports these features.
These three features have non-trivial interactions that need to be
accounted for, in particular when introducing properties on types, such as locations.

Let us consider the module shown in \cref{code:datatype}.
We declare a server datatype \ocamlc{t} with two parameters and we hide the definition in the signature.
We now want to check that \ocamlc{(t1, t2) t} is a correct type expressions.
However, without the type definition, we don't know if \ocamlc{t1} and \ocamlc{t2} are
base, client or server types. In order to type check the type sub-expressions, we
need more information about the definition of \ocamlc{t}.
The solution, much like variance, is to annotate type variables in datatypes with extra information.
%
This is done in the syntax for type declarations given in \cref{eliom:grammar}.
Each type parameters is annotated with a location. Type variables can only be used on the right location. This ensures proper separation of client and server type variables and their proper usage.

These annotations can be though as a simplistic kind system. One could
also considered \ocamlc{'a} as a constrained type variable, in the style of
\ml{}$^{\text{F}}$~\citep{MLF}.

\begin{ex}[!htb]
  \begin{subfigure}[b]{0.5\textwidth}
\begin{lstlisting}[language=eliom]
module M : sig
  type%server ('a, 'b) t
end = struct
  type%server ('a, 'b) t = 'a fragment * 'b
end
\end{lstlisting}\vspace{-4mm}
    \caption{Incorrect abstract datatype}
    \label[figure]{code:datatype:incorrect}
  \end{subfigure}~
  \begin{subfigure}[b]{0.55\textwidth}
\begin{lstlisting}[language=eliom]
module M : sig
  type%server ('a[@client], 'b) t
end = struct
  type%server ('a[@client], 'b) t = 'a fragment * 'b
end
\end{lstlisting}\vspace{-4mm}
    \caption{Correct abstract datatype}
    \label[figure]{code:datatype:correct}
  \end{subfigure}
  \caption{A module with an abstract datatype.}
  \cref{code:datatype:incorrect} does not exposes information about acceptable sides for \ocamlc{'a} and \ocamlc{'b}.
  In \cref{code:datatype:correct}, annotations specifying the side of type variables are exposed in the interface.
  \label{code:datatype}
  \vspace{-5mm}
\end{ex}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> theory/grammar.tex <==
% \begin{subfigure}{\linewidth}
% \begin{subfigure}[t]{0.48\linewidth}
%   \begin{align*}
%   \htag{Expressions}
%   e ::=&\ c\tag{Constant}\\
%   |&\ x_i\ |\ p.x \tag{Variables}\\
%   |&\ \Y\tag{Fixpoint}\\
%   |&\ \app{e}{e} \tag{Application}\\
%   |&\ \lam{x}{e} \tag{Function}\\
%   |&\ \letin{x}{e}{e}\tag{Let binding}\\
%   |&\ \cv{ e } \tag{\addedx{Fragments}}\\
%   |&\ \injf{x}{f} \tag{\addedx{Injections}}\\[2mm]
%   p ::=&\ X_i\ |\ p.X\ |\ \appm{p_1}{p_2}\tag{Path}\\
%   f ::= &\ p.x\ |\ x_i\ |\ c \tag{\addedx{Converter}}\\
%   c \in&\ \Const_\loc \tag{Constants}\\
%   \end{align*}
% \end{subfigure}~\hfill~
% \begin{subfigure}[t]{0.48\linewidth}
%   \begin{align*}
%   \htag{Type Expressions}
%     \tau ::=&\ \dots\\
%     |&\ p.t \tag{Path}\\
%     |&\ \alpha_{\added\loc}\tag{Type variables}\\
%     |&\ \cvtype{\tau} \tag{Fragment types}\\
%     |&\ \conv{\tau}{\tau} \tag{Converter types}\\
%   \htag{Module types}
%   M ::=&\ \dots\\
%   |&\ \functor[\sideX]{X_i}{\Mm_1}{\Mm_2}\tag{Mixed functor}\\
%   \htag{Signature components}
%   D ::=&\ \valm{x_i}{\tau}\\
%   |&\ \typem{\typicalt}{\tau}\\
%   |&\ \typeabsm{\typicalt}\\
%   |&\ \moduletym{X_i}{\Mm}
%   \end{align*}
% \end{subfigure}
% \caption{The expression language}
% \end{subfigure}

% \begin{subfigure}{\linewidth}
% \begin{subfigure}[t]{0.45\linewidth}
% \begin{align*}
%   \htag{Module Expressions}
%   \mm ::=&\ X_i\ |\ p.X\tag{Variables}\\
%   |&\ \constraint{\mm}{\Mm}\tag{Type constraint}\\
%   |&\ \appm{\mm_1}{\mm_2}\tag{Functor application}\\
%   |&\ \functor{X_i}{\Mm}{\mm}\tag{Functor}\\
%   |&\ \functor[\sideX]{X_i}{\Mm}{\mm}\tag{Mixed functor}\\
%   |&\ \struct{s}\tag{Structure}\\
%   \htag{Structure body}
%   \sm ::=&\ \emptym\ |\ \dm;\sm\\
%   \htag{Structure components}
%   \dm ::=&\ \letm{x_i}{e}\tag{Values}\\
%   |&\ \typem{\typicalt}{\tau}\tag{Types}\\
%   |&\ \modulem{X_i}{\mm}\tag{Modules}\\
%   \htag{Programs}
%   \Pm ::=&\ \prog{\sm}
% \end{align*}
% \end{subfigure}\hfill
% \begin{subfigure}[t]{0.5\linewidth}
% \begin{align*}
%   \htag{Module types}
%   \Mm ::=&\ \signature{\Sm}\tag{Signature}\\
%   |&\ \functor{X_i}{\Mm_1}{\Mm_2}\tag{Functor}
%   \addedrule{\\%
%     |&\ \functor[\sideX]{X_i}{\Mm_1}{\Mm_2}\tag{Mixed functor}\\
%   }%
%   \htag{Signature body}
%   \Sm ::=&\ \emptym\ |\ \Dm;\Sm\\
%   \htag{Signature components}
%   \Dm ::=&\ \valm{x_i}{\tau}\tag{Values}\\
%   |&\ \typem{\typicalt}{\tau}\tag{Types}\\
%   |&\ \typeabsm{\typicalt}\tag{Abstract types}\\
%   |&\ \moduletym{X_i}{\Mm}\tag{Modules}\\
%   \htag{Environments}
%     \Env ::=&\ \Sm
% \end{align*}
% \end{subfigure}
% \caption{The module language}
% \end{subfigure}

\input{theory/ml/grammar.tex}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> theory/ml/soa.tex <==
\subsection{Related works}\label{sec:ml:soa}

Our formalization of the expression language is inspired by
\citet{wright1994syntactic} which contains a small step semantics
for the core language and extensions for references and exceptions, along
with their soundness proofs. A discussion around the various styles of semantics
in the context of traces is also provided by \citet{CoIndTraces}.
%
The big step semantics takes inspiration from
\citet{DBLP:conf/esop/OwensMKT16} and \citet{DBLP:conf/popl/AminR17}.
\citet{Tofte88} also presents a big-step semantics for \ml
and proves the soundness in the context of polymorphic type inference.
A gentle introduction to soundness for big step semantics can be found
in \citet{SiekSoundness}.

The landscape of \ml modules is extremely rich, we only point to several
key work that are directly relevant.
Our module language is almost directly taken from \citet{Leroy94,Leroy95}
which is the basis of the \ocaml module language \citep{Ocamlmanual}.
The SML module system employs a different mechanism for propagating type
equalities based on a \ocamlc{sharing} annotation \citep{DefinitionSML}.
Such annotation does not lend itself immediately to separate compilation
\citep{DBLP:conf/ml/SwaseyVCH06}.
However, the SML module system has been (partially) mechanized
\citep{DBLP:conf/popl/LeeCH07}.
A thorough and very instructive comparison between the various modules
systems was done by \citet[Chapter 1 and 2]{dreyerthesis}.

The module system we presented here is expressed directly in term of the
syntax of the language. This is on purpose for two reasons. First, this
is how it is implemented in \ocaml, making it possible to reason
both about the formal system and the eventual implementation. Second, it
makes the various extensions of \eliom fairly easy to model. In particular,
we shall see that our compilation scheme for \eliom preserves the typing
relation. Such results would be more delicate to express if the module system
were expressed by elaboration.
However, if such constraints were not considered,
\cite{FingModules} define an \ml module system, including
first class modules and applicative functors, in term of System $F_\omega$.
This yields a simple yet feature-full system that could prove
easier to extend.

%   See \cite{wright1994syntactic},
%   \cite{DBLP:conf/popl/AminR17},
%   \cite{DBLP:conf/popl/LeeCH07},
%   \cite{DBLP:conf/esop/OwensMKT16},
%   \cite{Tofte88}.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../../main"
%%% End:


==> theory/module/compfunctor.tex <==
\begin{align*}
  \compile{c}{\modulem[\sideX]{x_i(x:M)\dots}{m};s}
  &=
    \modulem[]{x_i(x:\compile{c}{M})\dots}
    {\compile{c}{m}};\compile{c}{s}
\end{align*}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../../main"
%%% End:


==> theory/module/equivty.tex <==
\begin{mathpar}
  \inferrule
  { \bindingty[\loc']{\typicalt}{\tau} \in \Env \\
    \added{\canuseloc{\loc'}{\loc}}
  }
  { \equivty{\Env}{\appty{\tau_j^*}{t_i}}{\tau} }
  \and
  \inferrule
  { \wtm[\loc]{\Env}{p}
    {(\signature{S_1;\typem[\loc']{\typicalt}{\tau};S_2})} \\
    \added{\canuseloc{\loc'}{\loc}}
  }
  { \equivty{\Env}{\appty{\tau_j^*}{p.t}}{\substs{n_i}{p.n}{\bv{S_1}}{\tau}} }
\end{mathpar}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../../main"
%%% End:


==> theory/module/grammar.tex <==

\begin{subfigure}[t]{0.4\linewidth}
\begin{align*}
  \htag{Module Expressions}
  m ::=&\ x_i\ |\ p.x\ |\ \appm{m_1}{m_2}\ |\ \constraint{m}{M}\\
  |&\ \struct{s}\\
  |&\ \functor{x_i}{M}{m}\\
  |&\ \functor[\sideX]{x_i}{M}{m}\\
  \htag{Structure body}
  s ::=&\ \emptym\ |\ d;s\\
  \htag{Structure components}
  d ::=&\ \letm{v_i}{e_\loc}\\
  |&\ \typem{\typicalt}{\tau_\loc}\\
  |&\ \modulem{x_i}{m}\\
  \htag{Programs}
  P ::=&\ \prog{s}
\end{align*}
\end{subfigure}\quad
\begin{subfigure}[t]{0.4\linewidth}
\begin{align*}
  \htag{Module types}
  M ::=&\ \signature{S}\\
  |&\ \functor{x_i}{M_1}{M_2}\\
  |&\ \functor[\sideX]{x_i}{M_1}{M_2}\\
  \htag{Signature body}
  S ::=&\ \emptym\ |\ D;S\\
  \htag{Signature components}
  D ::=&\ \valm{v_i}{\tau_\loc}\\
  |&\ \typem{\typicalt}{\tau_\loc}\\
  |&\ \typeabsm{\typicalt}\\
  |&\ \moduletym{x_i}{M}
\end{align*}
\end{subfigure}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> theory/module/rcontexts.tex <==
% \begin{subfigure}[t]{0.25\linewidth}
% \begin{align*}
%   \htag{Client Contexts}
%   R ::=&\ \hole\ |\ \lam{x}{R}\\
%   |&\ \letin{v}{R}{e}\\
%   |&\ \letin{v}{e}{R}\\
%   |&\ \app{R}{e}\ |\ \app{e}{R}
% \end{align*}
% \end{subfigure}\qquad
% \begin{subfigure}[t]{0.5\linewidth}
\begin{align*}
  % \htag{Functor Contexts}
  R_f ::=&\ \hole\ |\ \appm{R_f}{m}\ |\ \appm{m}{R_f}
           \ |\ \functor[\sideX]{a}{M}{R_f}
  % \\
  % \htag{Module Contexts}
  % R_m ::=&\ \hole\ |\ \appm{R_m}{m}\ |\ \appm{m}{R_m}
  %          \ |\ \functor{x_i}{M}{R_m}\\
  % |&\ \struct{s;\ \letm[c]{v_i}{R};\ s'}\\
\end{align*}
% \end{subfigure}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../../main"
%%% End:


==> theory/module/rewriting.tex <==
\setlength{\jot}{-1pt}% Remove interline space in align*
% \textbf{Lifting of injections}
% \begin{mathpar}
%   \inferrule
%   { \text{$v$ is fresh.} }
%   { \rw[s]{\Env}
%     {\cv{\R{\injf{e}{f}}}}
%     {\letin{v}{e}{\cv{\R{\injf{v}{f}}}}}
%   }
%   \and
%   \inferrule
%   { \text{$v_i$ is fresh.} }
%   { \rw[\sideX]{\Env}
%     {\letm[c]{y}{\R{\injf{e}{f}}}}
%     {\begin{aligned}
%         &\letm[s]{v_i}{e};\\
%         &\letm[c]{y}{\R{\injf{v_i}{f}}}
%       \end{aligned}}
%   }
%   \and
%   \inferrule
%   { \text{$v_i$ is fresh.} }
%   { \rw[\sideX]{\Env}
%     {\modulem[c]{m_i}{\Rm{\injf{e}{f}}}}
%     {\begin{aligned}
%         &\letm[s]{v_i}{e};\\
%         &\modulem[c]{m_i}{\Rm{\injf{v_i}{f}}}
%       \end{aligned}}
%   }
% \end{mathpar}
%\textbf{Lambda lifting for mixed structures}
\begin{mathpar}
  \inferrule[Bind]
  { \text{$x_i'$ is fresh.} \\
    R_f \neq \hole\\
    \forall k.\ \functor[\sideX]{x_{i_k}:M_k}{m} \in R_f
  }
  { \rw[]{\Env}
    {\modulem[\sideX]{x_i}{\Rf{\struct{s}}}}
    {\begin{aligned}
        &\modulem[\sideX]{x_{i'}\overline{(x_{i_k}:M_k)}}{\struct{s}};\\
        &\modulem[\sideX]{x_i}{\Rf{x_{i'}\overline{(x_{i_k}:M_k)}}}
      \end{aligned}}
  }
  \and
  \inferrule[LiftUp]
  { \text{$x_i'$ is fresh}\\
    \{a\} = \bv{d}\\
    d' = alias(d)\\
    \widetilde{m} = \subst{a}{x'.a}{m}\\
    \widetilde{M} = \subst{a}{x'.a}{m}\\
    \wtm{\Env}{(\struct{d})}{M'}
  }
  { \rw[]{\Env}
    {\begin{aligned}
        &\mathtt{module}_\sideX\ x_j (x_a:M_a)\dots = \mathtt{struct}\\
        &\quad s;\\
        &\quad d;\\
        &\quad\modulem[\sideX]{x_i (x:M)}{m}\\
        &\quad s';\\
        &\mathtt{end}
      \end{aligned}}
    {\begin{aligned}
        &\mathtt{module}_\sideX\ x_j (x_a:M_a)\dots = \mathtt{struct}\\
        &\quad s;\\
        &\quad \modulem[\sideX]{x_i' (x': M') (x : \widetilde{M})}{\widetilde{m}};\\
        &\quad d;\\
        &\quad \modulem[\sideX]{x_i}{\appm{x_i'}{\struct{d'}}}\\
        &\quad s';\\
        &\mathtt{end}
      \end{aligned}}
  }
  \and
  \inferrule[LiftOut]
  { \text{$x_i''$ is fresh} }
  { \rw[]{\Env}
    {\begin{aligned}
        &\mathtt{module}_\sideX\ x_j (x_a:M_a) = \mathtt{struct}\\
        &\quad\modulem[\sideX]{x_i (x:M)}{m};\\
        &\quad s\\
        &\mathtt{end}
      \end{aligned}}
    {\begin{aligned}
        &\modulem[\sideX]{x_i' (x_a:M_a) (x:M)}{m};\\
        &\mathtt{module}_\sideX\ x_j (x_a:M_a) = \mathtt{struct}\\
        &\quad\modulem[\sideX]{x_i}{\appm{x_i'}{x_a}}\\
        &\quad s\\
        &\mathtt{end}
      \end{aligned}}
  }
\end{mathpar}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../../main"
%%% End:

